The Impact of Molecular Hydrogen Cooling on the Galaxy Formation Threshold

We study the impact of molecular (${\rm H_2}$) and atomic (HI) hydrogen cooling on the galaxy formation threshold. We calculate the fraction of dark matter (DM) halos that exceeds a critical mass required for star formation, $M_{\mathrm{crit}}(z)$, as a function of their peak mass. By convolving analytic halo mass accretion histories (MAHs) with models for $M_{\mathrm{crit}}(z)$, we predict that halos with peak virial masses below $\sim 10^8~M_{\mathrm{\odot}}$ can form stars before reionization through ${\rm H_2}$ cooling. These halos remain dark when only HI cooling and reionization are modeled. However, less than $\approx 10\%$ of halos with peak masses below $\sim 10^{7}~M_{\mathrm{\odot}}$ ever exceed $M_{\mathrm{crit}}(z)$, even when ${\rm H_2}$ cooling is included; this threshold is primarily set by relative streaming motion between DM and baryons imprinted at recombination. We obtain similar results using subhalo MAHs from an extremely high-resolution cosmological DM--only zoom-in simulation of a Milky Way (MW) analog (particle mass $6.3\times 10^3~M_{\mathrm{\odot}}$). Based on the abundance of MW satellites, these results imply that at least some known ultra-faint dwarf galaxies formed through ${\rm H_2}$ cooling. This work sharpens predictions for the galaxy formation threshold and demonstrates how its essential features emerge from the underlying distribution of halo growth histories.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

